Large $N$-ightmare Dark Matter

A dark QCD sector is a relatively minimal extension of the Standard Model (SM) that admits Dark Matter (DM) candidates but requires no portal to the visible sector beyond gravitational interactions: A "nightmare scenario" for DM detection. We consider a secluded dark sector containing a single flavor of light, vector-like dark quark gauged under $SU(N)$. In the large-$N$ limit, this single-flavor theory becomes highly predictive, generating two DM candidates whose masses and dynamics are described by few parameters: A light quark-antiquark bound state, the dark analog of the $\eta'$ meson, and a heavy bound state of $N$ quarks, the dark analog of the $\Delta^{++}$ baryon. We show that the latter may freeze-in with an abundance independent of the confinement scale, forming DM-like relics for $N \lesssim 10$, while the former may generate DM via cannibalization and freeze-out. We study the interplay of this two-component DM system and determine the characteristic ranges of the confinement scale, dark-visible sector temperature ratio, and $N$ that admit non-excluded DM, once the effects of self-interaction constraints and bounds on effective degrees of freedom at the BBN and CMB epochs are included.

==> afterenddoc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Large-$N$ arguments also imply that the interactions of the Boltzmann-suppressed $\deltaN$ with the $\etap$ plasma are exponentially suppressed in $N$, such that
%$\deltaN$'s may be produced out of thermal equilibrium  -- i.e. freeze-in -- by the thermal bath of $\etap$ via $\etap\etap\to\deltaN\bar\deltaN$. 
%The $\deltaN$ cosmological abundance $\Omega_\deltaN\sim e^{-2(c_* +1)N}$, with $c_*$ an ${\cal O}(1)$ parameter, which is independent of $\Lambda$,
%thus allowing for a significant cosmological $\deltaN$ abundance only for $N\lesssim10$. 
%%
%
%
%The cosmological abundance of the two stable species is controlled by two qualitatively different mechanisms: 
%On the one hand, $\deltaN$'s are produced out of thermal equilibrium (``freeze-in'') by the thermal bath of $\etap$ via $\etap\etap\to\deltaN\bar\deltaN$. 
%Because the cross section is exponentially suppressed in $N$, the $\deltaN$ cosmological abundance $\Omega_\deltaN\sim e^{-2(c_* +1)N}$, with $c_*$ an ${\cal O}(1)$ parameter, 
%thus allowing for a significant cosmological $\deltaN$ abundance only for $N\lesssim10$. 
%%The abundance of the $\etap$ is controlled by the interplay of $\etap\etap\to\deltaN\bar\deltaN$ and of the cannibal $2\etap\leftrightarrow4\etap$ processes. 
%We presented  that the large-$N$ relic density of $\etap$ scales like $\Omega_\etap\sim\Lambda^{26/20}N^{59/20}$.



%In that case, which we leave to future study, we expect a significantly different phenomenology, which includes the possibility of direct dark matter detection and of detection with particle colliders.


%The theory possesses two stable states: the lightest quark-antiquark meson (which we indicate as $\eta^\prime$), and the lightest bound state of $N$ quark in the color-singlet combination of the $N$ colors (which in analogy with the Standard Model we call $\Delta$). We use results from chiral perturbation theory and the large-$N$ limit of SU($N$) strongly-coupled theories to estimate the particle masses and the interaction cross sections responsible for the production of the two stable species in the early universe an for the species' self-interaction, which shape halos at late times. Ignorance about parameters entering these cross sections entail a certain degree of uncertainty in our predictions, which we study in detail.

%Production of the meson $\eta^\prime$ is dominated by 4-to-2 processes and by pair-annihilation into $\Delta$ pairs, while the $\Delta$ abundance is dominated by production out of thermal equilibrium (freeze in). We explain how the parameter space where the $\Delta$ is a viable dark matter candidate is largely independent of the confinement scale (with an upper limit where $\eta^\prime$'s become overabundant), and solely singles out a value for $N$ that corresponds to the right abundance. On the other hand, the abundance of the $\eta^\prime$ depends both on $\Lambda$ and on $N$ in a highly non-trivial way.

%The theory is constrained, besides by the abundance of its stable species', by the effect on self interactions, which generally rules out the $\Delta$ as a viable dark matter candidate (except for very large mass biases that make the $\Delta$ significantly more massive than the naive estimate $m_\Delta\sim N\Lambda$). In contrast, the $\eta^\prime$ generally sits at or below the level of self interaction that could be observationally detectable. In addition, if the ratio of the temperatures in the dark and visible sector is large enough, the theory predicts measurable effects on the effective number of relativistic degrees of freedom as constrained by CMB and BBN.

%A similar setup to what discussed here is one where the theory possesses an U$(N)$ group, with the $U(1)$ subgroup kinetically mixing with hypercharge. In that case, which we leave to future study, we expect a significantly different phenomenology, which includes the possibility of direct dark matter detection and of detection with particle colliders.


\begin{comment}
\subsection{$2\etap\to4\etap$ Cross Section}
The Lagrangian describing the number changing interactions of the dark $\eta'$ is given in Eqn.~(\ref{eqn:Letap}). Notice that there are two terms in the interaction Lagrangian that give contributions to $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$, one contribution from two four-point interaction vertices (see Fig.~(\ref{fig:two_four_eta_a})) and one from a single six-point interaction (see Fig.~(\ref{fig:two_four_eta_b}).) Both of the matrix elements for these diagrams have the same scaling with the parameters of the model. They can be written as:
\begin{align}
    \mathcal{A}_{a} & = \dfrac{256\pi^4\lambda_1^2m_{\etap}^6}{9\Lambda^8N^2}F_a(q_i\cdot q_j),   &
    \mathcal{A}_{b} & = -\dfrac{256\pi^4\lambda_2 m_{\etap}^6}{15\Lambda^8N^2}F_{b}(q_i\cdot q_j)
\end{align}
where $F_{a,b}$ are functions of scalar products of the external momenta scaled by the $\eta'$ mass: $q_{i} = p_{i}/m_{\eta'}$:
\begin{align}
    F_a &= \bigg{(}\frac{1}{Q\cdot Q - 1
    }
    (\qty(q_{1}\cdot Q)
   \qty(q_{2}\cdot q_{3})+
   \qty(q_{1}\cdot q_{3})
   \qty(q_{2}\cdot Q)+
   \qty(q_{1}\cdot q_{2}) 
   \qty(q_{3}\cdot Q))\\
   &\qquad\times(\qty(q_{4}\cdot Q)
   \qty(q_{5}\cdot q_{6})+
   \qty(q_{4}\cdot q_{6})
   \qty(q_{5}\cdot Q)+
   \qty(q_{4}\cdot q_{5}) 
   \qty(q_{6}\cdot Q))\bigg{)}\bigg{|}_{Q=q_4+q_5+q_6}\notag\\
   &\qquad + (\mathrm{permutations})\notag\\
   F_b &= 
   \qty(q_{1}\cdot q_{4}) \qty(q_{2}\cdot q_{6}) \qty(q_{3}\cdot q_{5})+
   \qty(q_{1}\cdot q_{2}) \qty(q_{3}\cdot q_{5}) \qty(q_{4}\cdot q_{6})+
   \qty(q_{1}\cdot q_{4}) \qty(q_{2}\cdot q_{5}) \qty(q_{3}\cdot q_{6})\notag\\
   &\quad +
   \qty(q_{1}\cdot q_{3}) \qty(q_{2}\cdot q_{6}) \qty(q_{4}\cdot q_{5})+
   \qty(q_{1}\cdot q_{2}) \qty(q_{3}\cdot q_{6}) \qty(q_{4}\cdot q_{5})+
   \qty(q_{1}\cdot q_{3}) \qty(q_{2}\cdot q_{5}) \qty(q_{4}\cdot q_{6})\notag\\
   &\quad +
   \qty(q_{1}\cdot q_{6}) [
    \qty(q_{2}\cdot q_{5}) \qty(q_{3}\cdot q_{4})+
    \qty(q_{2}\cdot q_{4}) \qty(q_{3}\cdot q_{5})+
    \qty(q_{2}\cdot q_{3}) \qty(q_{4}\cdot q_{5})
    ]\notag\\
   &\quad +
   \qty(q_{1}\cdot q_{5}) [
    \qty(q_{2}\cdot q_{6}) \qty(q_{3}\cdot q_{4})+
    \qty(q_{2}\cdot q_{4}) \qty(q_{3}\cdot q_{6})+
    \qty(q_{2}\cdot q_{3}) \qty(q_{4}\cdot q_{6})
    ]\notag\\
   &\quad +
   \qty(q_{5}\cdot q_{6}) [
    \qty(q_{1}\cdot q_{4}) \qty(q_{2}\cdot q_{3})+
    \qty(q_{1}\cdot q_{3}) \qty(q_{2}\cdot q_{4})+
    \qty(q_{1}\cdot q_{2}) \qty(q_{3}\cdot q_{4})
    ]
\end{align}
We can therefore write the squared matrix element for $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$ as:
\begin{align}
    |\cM(\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta')|^2 & =
    \qty(\dfrac{256\pi^4m_{\etap}^6}{\Lambda^8N^2})^2F(q_i\cdot q_j),\notag                                                             \\
    F(q_i\cdot q_j)                                        & = \qty[\lambda_1^4F_a^2 + \lambda_2^2F_b^2 - 2\lambda_1^2\lambda_2F_a F_b]
\end{align}
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[scale=0.2]{figures/two_four_eta_1.pdf}
        \caption{}
        \label{fig:two_four_eta_a}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[scale=0.2]{figures/two_four_eta_2.pdf}
        \caption{}
        \label{fig:two_four_eta_b}
    \end{subfigure}
    \caption{Example Feynman diagrams contributing to $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$. Note that there are many diagrams similar to the one shown in figure (a) that we have not shown.}\label{fig:two_four_eta}
\end{figure}
To compute the cross-section, we must evaluate the following integrals:
\begin{align}
    \sigma_{2\eta'\to4\eta'}(s) & = \qty(\dfrac{256\pi^4m_{\etap}^6}{\Lambda^8N^2})^2
    \dfrac{1}{2\sqrt{s}\sqrt{s-4m_{\eta'}^2}}
    \int
    d\Pi_{3}d\Pi_{4}d\Pi_{5}d\Pi_{6}
    F(q_{i}\cdot q_{j})
    \delta^4\left(P-\sum_{i=1}^4 p_i\right)
\end{align}
where $d\Pi_i = \frac{d^3p_{i}}{(2\pi)^32E_i}$ and $P = p_{1} + p_2$ is the sum of the initial state momenta. As we did with the matrix element, we will factor out the mass dimensions of the invariant phase space integral by defining $q_i = p_i/m_{\eta'}$, $\epsilon_i = E_i / m_{\eta'}$ and $z = \sqrt{s}/m_{\eta'}$. Then, we can write the cross section as:
\begin{align}
    \sigma_{2\eta'\to4\eta'}(s) & = \qty(\dfrac{256\pi^4m_{\etap}^7}{\Lambda^8N^2})^2
    \bar{\sigma}(z)
\end{align}
with
\begin{align}
    \bar{\sigma}(z) & =
    \dfrac{1}{2z\sqrt{z^2-4}}
    \int
    \frac{d^3q_{3}}{(2\pi)^32\epsilon_3}
    \frac{d^3q_{4}}{(2\pi)^32\epsilon_4}
    \frac{d^3q_{5}}{(2\pi)^32\epsilon_5}
    \frac{d^3q_{6}}{(2\pi)^32\epsilon_6}
    F(q_{i}\cdot q_{j})\delta\left(Q-\sum_{i=1}^{4}q_i\right)
\end{align}
To evaluate $\bar{\sigma}$, we using the simple Monte Carlo phase-space generator {\bf{RAMBO}}\cite{kleiss1985new} and verify our results using {\bf{MadGraph}}\cite{alwall2011madgraph}. The numerical values of $\bar{\sigma}(z)$ are shown in Fig.~(\ref{fig:eta_cs}). With the numerical cross section in hand, we can numerically evaluate the thermally-average annihilation cross section, given by:
\begin{align}\label{eqn:thermal_average_22}
    \expval{\sigma_{2\eta'\to4\eta'} v} & =
    \qty(\dfrac{256\pi^4m_{\etap}^7}{\Lambda^8N^2})^2
    \dfrac{x}{4K^2_{2}(x)}
    \int_{4}^{\infty} dz z^2(z^2-4)K_{1}(xz)\bar{\sigma}(z)
\end{align}
with $x = m_{\eta'} / T$. Using detailed balance, it is simple to compute the thermally-averaged cross section for the reverse process $\expval{\sigma_{4\etap\to2\etap}v}$:
\begin{align}\label{eqn:thermal_average_22}
    \expval{\sigma_{4\eta'\to2\eta'} v^3} & = \dfrac{1}{n^2_{\etap,\mathrm{eq}}}\expval{\sigma_{2\eta'\to4\eta'} v}
\end{align}
Fig.~(\ref{fig:eta_tcs}) displays an example thermally-average cross section for $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$.

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/eta_cs.pdf}
        \caption{}
        \label{fig:eta_cs}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/eta_tcs.pdf}
        \caption{}
        \label{fig:eta_tcs}
    \end{subfigure}
    \caption{(left) Contributions from the 4-pt and 6-pt terms of the chiral Lagrangian to the zero-temperature cross section for $2\etap\to4\etap$ with all model dependent pre-factors removed. (right) Rescaled thermally-averaged cross section for $2\etap\leftrightarrow4\etap$ with $\lambda_1 = 1/10$ and $\lambda_2=1$.}\label{fig:eta_zt_cs_tcs}
\end{figure}

\subsection{Computing the Dark Temperature}

As mentioned in the previous section, we parameterize the ratio of the dark temperature, $T_{d}$, to the SM temperature, $T_{\SM}$ as: $\xi = T_{d} / T_{\SM}$. The evolution of $\xi$ can be determined given some initial value, denoted as $\xi_{\mathrm{inf}} = T_{d,\mathrm{inf}} / T_{\SM,\mathrm{inf}}$, specified for instance after inflation. For our purposes, we take $\xi_{\mathrm{inf}}$ to be a free parameter. Assuming that there is no significant entropy exchange between the two sectors, the ratio of the dark entropy density, $s_{d}$ to the SM entropy density, $s_{\SM}$ should remain constant. Right after inflation, this ratio is:
\begin{align}
    \dfrac{s_{d,\mathrm{inf}}}{s_{\mathrm{inf}}} = \dfrac{g^{d}_{*S,\mathrm{inf}}}{g^{\SM}_{*S,\mathrm{inf}}}\xi^{3}_{\mathrm{inf}}.
\end{align}
Here $g^{\SM}_{*S,\mathrm{inf}}\sim 106.75$ and $g^{d}_{*S,\mathrm{inf}}$ counts the number of degrees of freedom in the dark sector, which at high temperatures, contains the dark gluons and dark quarks and potentially a dark photon. Thus,
\begin{align}
    g^{d}_{*S,\mathrm{inf}} &= \dfrac{7}{8}\cdot 4N + 2(N^2 - 1)
\end{align}
where $(7/8)\cdot 4N$ counts the number of degrees of freedom from the dark quarks and $2(N^2 - 1)$ counts the number of degrees of freedom in dark gluons. After confinement, the number of degrees of freedom in the dark sector sharply drops. From lattice simulations, the phase transition temperature has been estimated to be roughly $\Lambda/2$. Since the mass of the dark $\Delta$-baryon is $N\Lambda$, it will be non-relativistic for $T_{d} < \Lambda/2$. To compute the evolution of $\xi$, we need to solve the following:
\begin{align}
    \xi^3 = \dfrac{h_{\SM}(T_{\mathrm{SM}})}{h_{\SM,\infty}}\dfrac{h_{d,\infty}}{h_{d}(\xi T_{\mathrm{SM}})}\xiinf^{3}
\end{align}
To compute $h_{d}(T_{d})$, we use the expressions given in Appendix~(\ref{app:equilibrium_quant}). In general, this equation has no analytic solution. In order to solve the equation, we use a bracketing root finding algorithm. In order to bracket the root, we first isolate all of the $\xi$-dependence on one side:
\begin{align}\label{eqn:xi_root_eqn}
    \xi^3h_{d}(\xi T_{\mathrm{SM}}) = \dfrac{h_{\SM}(T_{\mathrm{SM}})h_{d,\infty}}{h_{\SM,\infty}}\xiinf^{3}
\end{align}
For a fixed value of $T$, the right-hand-side is a constant. We note that the left-hand-side is an injective function from the positive reals to the positive reals. We can additionally bound this function above and below by injective functions, using the following:
\begin{align}
    \mathrm{max}\left(\xi^{3}g_{\gamma}, g_{\eta}\dfrac{45x_{\mathrm{SM}}^{5/2}}{4\sqrt{2}\pi^{7/2}}e^{-x_{\mathrm{SM}}/\xi}\sqrt{\xi}\right) < \xi^{3}h_{d}(\xi T_{\mathrm{SM}}) < \xi^{3}\left(g_{\eta} + \dfrac{7}{8}g_{\Delta}\right),
\end{align}
Additionally, $x_{\mathrm{SM}} = m_{\etap}/T_{\mathrm{SM}}$. These bounds can be derived by taking the ultra-relativistic and non-relativistic limits of the expression for $h_{d}$. Note that for the lower bound, we have taken only the largest contribution in the non-relativistic limit (any additional terms will only make the expression larger.) Both sides of the inequalities are monotonically increasing functions of $\xi$. Thus, if we can find where the bounding functions cross the RHS of Eqn.~(\ref{eqn:xi_root_eqn}), we can find a bounds on the value of $\xi$.
Upper and lower bounds on $\xi$ are given by:
\begin{align}
    \left(\dfrac{h_{\SM}(T_{\mathrm{SM}})h_{d,\infty}}{(7g_{\Delta}/8+g_{\eta})h_{\SM,\infty}}\right)^{1/3}\xiinf< \xi(T_{\mathrm{SM}}) < \dfrac{2x_{\mathrm{SM}}}{W\left(2x_{\mathrm{SM}}/D^2\right)}
\end{align}
where 
\begin{align}
    D &= g_{\eta}\dfrac{h_{\SM}(T_{\mathrm{SM}})h_{d,\infty}}{h_{\SM,\infty}}\left(\dfrac{45x_{\mathrm{SM}}^{5/2}}{4\sqrt{2}\pi^{7/2}}\right)^{-1}\xiinf^3
\end{align}
where $W(x)$ is the Lambert-W function, i.e. the inverse of $f(x)=xe^{x}$. %If instead we include the dark photon, the bounds become:
%\begin{align}
%     \left(\dfrac{h_{\SM}(T)h_{d,\infty}}{(7g_{\Delta}/4+g_{\eta} + g_{\gamma})h_{\SM,\infty}}\right)^{1/3}\xiinf< \xi < \left(\dfrac{h_{\SM}(T)h_{d,\infty}}{g_{\gamma}h_{\SM,\infty}}\right)^{1/3}\xiinf
%\end{align}
%In both cases, 
The value of $\xi$ gets close (but not equal) to the lower bound for large SM temperatures and asymptotically approaches the upper bound as the SM temperature tends to zero. %In the case of no dark photon, 
$\xi$ will continue to increase without bound until all dark particles have frozen out. In our scenario, the $\etap$ is the last to freeze-out. When it does, the temperature of the $\etap$ will cease to increase and will redshift as:
\begin{align}
    \xi \sim \xi_{\mathrm{f.o.}}\dfrac{T_{\mathrm{SM}}}{T_{\mathrm{SM,f.o.}}}
    \qquad \mathrm{or} \qquad
    T_{d} \sim T_{d,\mathrm{f.o.}}\left(\dfrac{T_{\mathrm{SM}}}{T_{\mathrm{SM,f.o.}}}\right)^2
\end{align}
Due to the fact that the dark sector temperature can exponentially increase with respect to the SM temperature, it becomes important to consider the effects of the dark sector on the total energy density to the Universe and its effects on the Hubble rate. We write the total energy density of the Universe as a function of the SM temperature as:
\begin{align}
    \rho_{\mathrm{tot}}(T_{\SM}) &= \dfrac{\pi^2}{30}g_{\mathrm{eff}}T_{\SM}^4
\end{align}
where, the effective degrees of freedom stored in energy, $g_{\mathrm{eff}}$, is given by:
\begin{align}\label{eqn:geff}
    g_{\mathrm{eff}}(T_{\SM}) = g_{\SM}(T_{\SM}) + g_{d}(\xi T_{\SM}) \xi^4(T_{\SM})
\end{align}
Then, the Hubble rate is given by:
\begin{align}\label{eqn:hubble_rate}
    H(T_{\SM}) &= \dfrac{T_{\SM}^2}{M_{\mathrm{pl}}}\sqrt{\dfrac{8\pi^3}{90} g_{\mathrm{eff}}}
\end{align}
where $M_{\mathrm{pl}} = 1.221\times10^{19} \ \mathrm{GeV}$ is the Planck mass.




\subsection{Solving the Boltzmann Equations}
The fully-coupled Boltzmann equations describing the evolution of the comoving number densities of the $\etap$ and $\deltaN$ are given in Eqn.~(\ref{eqn:boltzeta}) and Eqn.~(\ref{eqn:boltzeta}). Given that the phase-transition occurs at a dark temperature $T_{d}\sim \Lambda / 2$, the $\Delta$ will in general be very cold after the dark QCD phase-transition. We thus assume that the initial $\Delta$ abundance is essentially zero. This allows use to neglect the back-reactions between the $\etap$ and $\deltaN$, i.e. the $\deltaN\bar{\deltaN}\to\etap\etap$ collision term. For ease of controlling numerical errors, we convert the differential equation for $Y_{\etap}$ into an equation for $W_{\etap} = \ln(Y_{\etap})$. Thus, the equations we solve are:
\begin{align}
\dv{W_{\etap}}{\ln(x_{\SM})}
	 & = - \sqrt{\frac{\pi}{45}}M_{\mathrm{pl}}g^{1/2}_{\mathrm{eff},*} T_{\mathrm{SM}}s^2_{\SM} \expval{\sigma_{4\etap \to 2\etap} v^3} e^{W_{\etap}}\qty[e^{2W_{\etap}} - e^{2W_{\etap,\mathrm{eq}}}] \,,\\
\dv{Y_{\deltaN}}{x_{\SM}}
	& = \sqrt{\frac{\pi}{45}}\dfrac{M_{\mathrm{pl}}g^{1/2}_{\mathrm{eff},*}}{x_{\mathrm{SM}}}\expval{\sigma_{\etap\etap \to  \deltaN \deltaNb} v } e^{2W_{\etap}}\\
\end{align}
where
\begin{align}
    g^{1/2}_{\mathrm{eff},*} \equiv \qty(1 + \dfrac{T_{\mathrm{SM}}}{3h_{\mathrm{SM}}}\dv{h_{\mathrm{SM}}}{T_{\mathrm{SM}}})\dfrac{h_{\mathrm{SM}}}{\sqrt{g_{\mathrm{SM}}}}
\end{align}
To solve these equations, we use the variable order, implicit, stiff-ODE solver {\bf{radau}}\cite{hairer1999stiff}\footnote{This code is available from \url{https://unige.ch/~hairer/software.html}.} converted from FORTRAN to {\bf{c++}} using {\bf{f2c}}\cite{feldman1990fortran}.
\end{comment}
\clearpage






\section{Results}\label{sec:results}

We present out results in the plane defined by $\Lambda$ and $N$, and in that defined by the self-interaction cross section over mass, versus mass. We shade in blue the regions on the plane where self-interaction cross sections over mass exceed the limits of 1 barn/GeV, and in tan the region corresponding to self-interaction cross sections over mass are within 1.5 orders of magnitude of 1 barn/GeV. The planes show with dashed red lines the parameters corresponding to the $\Delta$ having a relic abundance $\Omega_\Delta h^2\sim0.12$, and with dot-dashed (in the left panels) and solid (right panels) blue lines the parameters corresponding to where the $\eta^\prime$ relic abundance is $\Omega_{\eta^\prime} h^2\sim0.12$.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/side_by_side_bm.pdf}
    \caption{Contours where the combined relic densities (solid black) of the $\eta'$ and $\Delta$ equal the observed DM relic density of $\Omega_{\mathrm{CDM}} h^2\sim0.12$. The red, dashed-dotted and purple, dashed contours shows where the $\Delta$ and $\eta'$ individually produce the correct relic density. The solid blue regions show where the self interaction (weighted by the relic densities - see text) are larger than $\sigma/m\gtrsim0.1 \ \mathrm{cm}^2/\mathrm{g}$.}
    \label{fig:benchmark}
\end{figure}
In each figure we study the impact of changing one of the theory's ``nuisance parameters'' at a time, while the concluding figure \ref{fig:final} summarizes the range spanned by all parameters in one single figure. We start, in fig.~\ref{fig:benchmark}, with our baseline benchmark choices: as indicated in the left panel, we set $L_1=1$, $c=1$, $a=1$, $\mu_\eta=\mu_\Delta=1$, and assume a ratio of dark-to-visible sector temperatures $\xiinf=10^-2$. The left panel illustrates a result we anticipated analytically above, which is that the $\Delta$ relic abundance is entirely controlled by $N$, once the critical $c$ parameter is fixed. Secondly, the panel shows how for our benchmark parameter choice, the dark matter can only be made out of $\eta^\prime$s, with $N\gg10$. The right panel, finally, shows that the preferred range of  $\eta^\prime$ masses is between a few keV (for very large $N$) up to around 1 MeV, when self-interaction constraints and an excessive relic density set an upper limit to the dark matter mass in this model.



\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/side_by_side_c.pdf}
    \caption{Same as in fig.~\ref{fig:benchmark}, but for $c=1/2$ (top panels) and $c=3/2$ (bottom panels); we also show with a grey dashed line the benchmark case ($c=1$).}
    \label{fig:c}
\end{figure}
In the following figure \ref{fig:c}, we vary the parameter $c$, which effective controls the probability for one of the $N$ dark quarks in the $\Delta$ to annihilate with an antiquark from the $\bar\Delta$ ($c=-\log p$ as indicated above). A suppression in the value of $c$ naturally yields a larger needed $N$, since the $\bar\Delta\Delta$ cross section scales like $e^{-cN}$; this is illustrated in the left panels, where in the top $c=1/2$, needing a larger $N$ and in the bottom $c=3/2$, needing a smaller $N$ too achieve the right thermal relic abundance. As anticipated, the value of $c$ doe snot impact the $\eta^\prime$ phenomenology. The impact of $c$ on the $\sigma_{\rm SI}/m$ plane is limited to the turning point where the relic density of the $\Delta$ dominates over that of the $\eta^\prime$, and as a result allows for slightly larger $\eta^\prime$ masses for larger $c=3/2$; such larger values are in tension with the self-interaction constraints.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/side_by_side_l1.pdf}
    \caption{Same as in fig.~\ref{fig:benchmark}, but for $L_1=10^{-3}$ (top panels) and $L_1=10$ (bottom panels); we also show with a grey dashed line the benchmark case ($L_1=1$).}
    \label{fig:L1}
\end{figure}
Fig.~\ref{fig:L1} shows the impact of the $L_1$ parameter, which controls 2-to-2 $\eta^\prime$ processes. We allow for a very large range of values, assuming $L_1=10^{-3}$ in the top panels, and $L_1=10$ in the bottom panels. While the $L_1$ parameter has a relatively minimal and indirect impact on the relic density, it directly controls the $\eta^\prime$ self interactions, which scales with $L_1^2$. This is directly reflected in the right panels, where a suppressed value of $L_1$ makes the $\eta^\prime$ self interaction very suppressed, and vice verse for a larger value, which makes self interactions generically in tension with observations. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/side_by_side_mu_eta.pdf}
    \caption{Same as in fig.~\ref{fig:benchmark}, but for $\mu_\eta=1/2$ (top panels) and $\mu_\eta=3/2$ (bottom panels); we also show with a grey dashed line the benchmark case ($\mu_\eta=1$).}
    \label{fig:mueta}
\end{figure}
The following fig.~\ref{fig:mueta} studies the effect of changing the mass ``renormalization'' parameter $\mu_{\eta^\prime}$: as shown in Eq.~(ref{eq:selfinteta}), the mass dependence explicitly appears in the self-interaction cross section; As above, the impact on the relic density is minimal, while that on the self-interaction cross section (right panels) quite significant, $\sigma/m\sim \mu_{\eta^\prime}^7$.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/side_by_side_mu_delta.pdf}
    \caption{Same as in fig.~\ref{fig:benchmark}, but for $\mu_\Delta=1/2$ (top panels) and $\mu_\Delta=3/2$ (bottom panels); we also show with a grey dashed line the benchmark case ($\mu_\Delta=1$).}
    \label{fig:muDelta}
\end{figure}
A qualitative difference appears in the case of the $\Delta$ (fig.~\ref{fig:muDelta}): here the thermal relic density is quite heavily impacted by a suppression or enhancement of the $\Delta$ mass (left panels); the impact on the self-interaction cross section (right panels) is instead limited. In either case, the range of viable dark matter models is unchanged, with the $\eta^\prime$ remaining the only viable candidate over the identical mass range.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/side_by_side_xi_inf.pdf}
    \caption{Same as Fig.~(\ref{fig:benchmark}) but with $\xiinf= 10^{-1}$ (top), $\xiinf= 5\times 10^{-2}$ (middle) and $10^{-1}$ (bottom). The yellow and the red regions show where $\Delta N_{\mathrm{eff}}(T_{\mathrm{BBN}})$ and $\Delta N_{\mathrm{eff}}(T_{\mathrm{CMB}})$ are larger than $0.3$.}
    \label{fig:xi_inf_sens}
\end{figure}
The last figure shows the impact of changing the dark-to-visible sector asymptotic temperature ratio $\xiinf$. First, in the top panel, we set $\xiinf=10^{-3}$: such ``cold'' dark sector actually allows for the $\Delta$ to be a viable dark matter candidate, and suppresses the $\eta^\prime$ self interaction rate to levels that could not conceivably be probed with observations. A colder dark sector implies both larger values of $\Lambda$ and smaller values of $N$, rendering the mass of the $\eta^\prime$, which scales like $\Lambda/\sqrt{N}$, significantly larger, up to a few GeV.

A ``hotter'' dark sector, as in the middle ($\xiinf=5\times 10^{-2}$) and bottom ($\xiinf=0.1$) panels, implies, as expected, much more stringent constraints from measures of non-standard relativistic degrees of freedom at CMB and BBN. Additionally, a hotter dark sector also forces larger values of $N$ and smaller values of $\Lambda$, suppressing the mass of the $\eta^\prime$ and enhancing constraints from self-interactions. We find that this scenarios is completely ruled out unless $\xiinf\ll0.1$.

\begin{figure}
    \centering
    \mbox{\includegraphics[width=0.55\textwidth]{figures/lam_n_combined.pdf} \includegraphics[width=0.55\textwidth]{figures/si_vs_m_combined.pdf}}
    \caption{Left: The range of values in the ($N,\Lambda$) plane  compatible with thermal relic dark matter spanned when ``nuisance parameters'' are varied as discussed in the text; the solid line corresponds to our benchmark;  Right: the predictions on the $\sigma_{\rm SI}/m$ versus mass plane for a generous span of  ``nuisance parameters''; solid and dashed lines correspond to the $\eta^\prime$ and $\Delta$.}
    \label{fig:combined}
\end{figure}
Our final summary plots in Fig.~\ref{fig:combined} visually show the range of values in the ($N,\Lambda$) plane covered by models with the right relic abundance (we do not show constraints as those depend on the nuisance parameters we vary). The maximal variations for the region where the $\Delta$ is the dark matter stems from the parameter $\mu_\Delta$, while in the $\eta^\prime$ is due to the ratio of dark-to-visible sector temperature. In the right panel, we show the effect of the nuisance parameters on the $\sigma_{\rm SI}/m$ versus mass plane. Here, the most important effects stem from $L_1$ and $\xiinf$ for the $\eta^\prime$, while the effect of the nuisance parameters is quite minimal for the $\Delta$.








\section{Discussion and Conclusions}\label{sec:conclusions}
We studied a single flavor strongly-coupled, completely secluded composite dark matter model with gauge group SU($N$), in the large $N$ limit. The theory is in principle fully defined by the choice of the confinement scale $\Lambda$, $N$, and the ratio of the dark-to-visible sector temperature (we choose to indicate this ratio with the value it has at asymptotically large temperatures, and we call it $\xiinf$).

The theory possesses two stable states: the lightest quark-antiquark meson (which we indicate as $\eta^\prime$), and the lightest bound state of $N$ quark in the color-singlet combination of the $N$ colors (which in analogy with the Standard Model we call $\Delta$). We use results from chiral perturbation theory and the large-$N$ limit of SU($N$) strongly-coupled theories to estimate the particle masses and the interaction cross sections responsible for the production of the two stable species in the early universe an for the species' self-interaction, which shape halos at late times. Ignorance about parameters entering these cross sections entail a certain degree of uncertainty in our predictions, which we study in detail.

Production of the meson $\eta^\prime$ is dominated by 4-to-2 processes and by pair-annihilation into $\Delta$ pairs, while the $\Delta$ abundance is dominated by production out of thermal equilibrium (freeze in). We explain how the parameter space where the $\Delta$ is a viable dark matter candidate is largely independent of the confinement scale (with an upper limit where $\eta^\prime$'s become overabundant), and solely singles out a value for $N$ that corresponds to the right abundance. On the other hand, the abundance of the $\eta^\prime$ depends both on $\Lambda$ and on $N$ in a highly non-trivial way.

The theory is constrained, besides by the abundance of its stable species', by the effect on self interactions, which generally rules out the $\Delta$ as a viable dark matter candidate (except for very large mass biases that make the $\Delta$ significantly more massive than the naive estimate $m_\Delta\sim N\Lambda$). In contrast, the $\eta^\prime$ generally sits at or below the level of self interaction that could be observationally detectable. In addition, if the ratio of the temperatures in the dark and visible sector is large enough, the theory predicts measurable effects on the effective number of relativistic degrees of freedom as constrained by CMB and BBN.

A similar setup to what discussed here is one where the theory possesses an U$(N)$ group, with the $U(1)$ subgroup kinetically mixing with hypercharge. In that case, which we leave to future study, we expect a significantly different phenomenology, which includes the possibility of direct dark matter detection and of detection with particle colliders.




\appendix
\section{Equilibrium Quantities}\label{app:equilibrium_quant}
In this appendix, we review the equilibrium quantities that arise in cosmology: the number, energy, pressure and entropy densities. The exact expressions for these quantities are:
\begin{align}
    n_i(T) &= \dfrac{g_iT_i^3}{2\pi^2}x_{i}^3\int_{1}^{\infty}\dfrac{y\sqrt{y^2-1}}{\exp(yx_i)-\eta_{i}}dy\\
    \rho_{i}(T_{d}) & = \dfrac{g_{i}T_i^4}{2\pi^2}x_i^4\int_{1}^{\infty}\dfrac{y^2\sqrt{y^2-1}}{\exp(yx_i)-\eta_{i}}dy\\
    P_{i}(T_{d}) & = \dfrac{g_{i}T_i^4}{6\pi^2}x_{i}^4\int_{1}^{\infty}\dfrac{(y^2-1)^{3/2}}{\exp(yx_{i})-\eta_{i}}dy\\
    s_{i}(T_{d}) &=
    \dfrac{g_{i}T_i^3}{2\pi^2}x_{i}^3\int_{1}^{\infty}\dfrac{y^2\sqrt{y^2-1} + \frac{1}{3}(y^2-1)^{3/2}}{\exp(yx_{i})-\eta_{i}}dy
\end{align}
where the subscript $i$ labels the particular particle, $x_{i} = m_{i} /T_{i}$ where $m_{i}$ and $T_{i}$ are the mass and temperature of the particle, $g_{i}$ is the number of degrees of freedom and $\eta_{i} = 1$ for bosons and $\eta_{i} = -1$ for fermions. We can evaluate these integrals using the following:
\begin{align}
    \dfrac{1}{e^{yx}-\eta} = \dfrac{e^{-xy}}{1-\eta e^{-xy}} = e^{-xy}\sum_{n=0}^{\infty}\left(\eta e^{-xy}\right)^n = \sum_{n=0}^{\infty}\eta^{n}e^{-(1+n)xy}
\end{align}
Using this, we find that:
\begin{align}
    n_{i}(T_{i}) &= \dfrac{g_{i}T_i^3}{2\pi^2}x_{i}^2\sum_{n=0}^{\infty}\dfrac{\eta^{n}}{1+n}K_{2}[(1+n)x_{i}]\\
    \rho_{i}(T_{i}) &= \dfrac{g_{i}T_i^4}{2\pi^2}x_{i}^2\sum_{n=0}^{\infty}\dfrac{\eta^{n}}{(1+n)^2}\left((1+n)x_{i}K_{1}[(1+n)x_{i}]+3K_{2}[(1+n)x_{i}]\right)\\
    P_{i}(T_{i})
    &= \dfrac{g_{i}T_i^4}{2\pi^2}x_{i}^2\sum_{n=0}^{\infty}\dfrac{\eta^{n}}{(1+n)^2}K_{2}[(1+n)x_{i}]\\
    s_{i}(T_{i})
    &= \dfrac{g_{i}T_d^3}{2\pi^2}x_{i}^3\sum_{n=0}^{\infty}\dfrac{\eta^{n}}{(1+n)}K_{3}[(1+n)x_{i}]
\end{align}
If we have a set of many particles in thermal equilibrium, then the total energy and entropy densities are:
\begin{align}
    \rho(T) &= \dfrac{\pi^2}{30}g_{\mathrm{eff}}(T)T^{4}\\
    s(T) &= \dfrac{2\pi^2}{45}h_{\mathrm{eff}}(T)T^{3}
\end{align}
where $g_{\mathrm{eff}}$ and $h_{\mathrm{eff}}$ are the effective numbers of degrees of freedom stored in energy and entropy, given by:
\begin{align}
    g_{\mathrm{eff}}(T) &= \sum_{i}\left(\dfrac{T_i}{T}\right)^4\dfrac{30g_{i}}{2\pi^4}x_{i}^2\sum_{n=0}^{\infty}\dfrac{\eta^{n}}{(1+n)^2}\left((1+n)x_{i}K_{1}[(1+n)x_{i}]+3K_{2}[(1+n)x_{i}]\right)\\
    h_{\mathrm{eff}}(T) &= \sum_{i}\left(\dfrac{T_{i}}{T}\right)^3\dfrac{45g_{i}}{4\pi^4}x_{i}^3\sum_{n=0}^{\infty}\dfrac{\eta^{n}}{(1+n)}K_{3}[(1+n)x_{i}]
\end{align}


\section{Boltzmann Equation}
Recall that the Boltzmann equation takes the following form:
\begin{align}
    L[f] = C[f]
\end{align}
where $L[f]$ is the Liouville operator and $C[f]$ is the collision operator describing number changing processes. In the NR limit with a homogeneous and isotropic universe, the Liouville operator can be written as:
\begin{align}
    L[f] = E\dfrac{\partial f}{\partial t} - \dfrac{\dot{a}}{a}|\vec{p}|^2\dfrac{\partial f}{\partial E}
\end{align}
If we integrate the Liouville operator over phase space, we find
\begin{align}
    g\int \dfrac{d^3p}{(2\pi)^3}L[f] = \dfrac{dn}{dt} + 3Hn
\end{align}
Similarly, integrating over the

\section{Thermally-Averaged Cross-Sections}\label{app:thermal_averages}
In this appendix, we describe how to compute the thermally-average cross sections for the number changing interactions involving the dark $\eta'$ meson and dark $\Delta$ baryon. The dark $\eta'$ meson can change its number density through two interactions: $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$ or $\eta'\eta'\leftrightarrow\bar{\Delta}\Delta$ while the dark $\Delta$ baryon changes its number density through the later of these interactions. 

The computation for a $AB\to X$ (with $X$ being any final state) thermally-average cross section is well known. It can be written as:
\begin{align}
    \expval{\sigma(AB\to X) v} &= \dfrac{\int \frac{d^3p_A}{(2\pi^3)} \frac{d^3p_B}{(2\pi^3)}f_{\mathrm{eq}}(E_A,T)f_{\mathrm{eq}}(E_B,T) \sigma(AB\to X) v_{\mathrm{M\o l}}}{\int \frac{d^3p_A}{(2\pi^3)} \frac{d^3p_B}{(2\pi^3)}f_{\mathrm{eq}}(E_A,T)f_{\mathrm{eq}}(E_B,T)}
\end{align}
where $f_{\mathrm{eq}}(E_i, T)$ is the equilibrium phase-space density for the incoming particles and $v_{\mathrm{M\o l}}$ being the M{\o}ller velocity: $v_{\mathrm{M\o l}} = \sqrt{(p_A\cdot p_B)-m_A^2m_B^2}/E_AE_B$. In the case where the two initial particles are identical and taking $f_{\mathrm{eq}}(E,T)=e^{-E/T}$, the expression for the thermally-average cross section reduces to:
\begin{align}\label{eqn:thermal_average_22}
    \expval{\sigma v} &= \dfrac{2\pi^2T\int_{4m^2}^{\infty} ds \sqrt{s}(s-4m^2)K_{1}(\sqrt{s}/T)\sigma(s)}{\left(4\pi m^2 TK_{2}(m/T)\right)^2}
\end{align}
This is the expression we will be evaluating in the remaining subsections. We note that, after obtaining an expression for $\expval{\sigma(\eta'\eta'\to\eta'\eta'\eta'\eta') v}$, we can obtain the thermally-averaged cross section for the reverse process using detailed balance.

\subsection{$\eta'\eta'\leftrightarrow \eta'\eta'\eta'\eta'$}
The Lagrangian describing the number changing interactions of the dark $\eta'$ is given in Eqn.~(\ref{eqn:eta_int_lag}). Notice that there are two terms in the interaction Lagrangian that give contributions to $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$, one contribution from two four-point interaction vertices (see Fig.~(\ref{fig:two_four_eta_a})) and one from a single six-point interaction (see Fig.~(\ref{fig:two_four_eta_b}).) Both of the matrix elements for these diagrams have the same scaling with the parameters of the model. They can be written as:
\begin{align}
    \cM_{a} &= \dfrac{L_{1}^2m_{\eta'}^6}{f_{\eta'}^4\Lambda^4}F_{a}(q_i\cdot q_j), &
    \cM_{b} &= \dfrac{L_{2}m_{\eta'}^6}{f_{\eta'}^4\Lambda^4}F_{b}(q_i\cdot q_j)
\end{align}
where $F_{a,b}$ are functions of scalar products of the external momenta scaled by the $\eta'$ mass: $q_{i} = p_{i}/m_{\eta'}$. Since we only know the scaling of various parameters of theory with $N$ and $\Lambda$ (i.e. we don't know the exact numerical prefactors/values) we will neglect the contribution from the six-point interaction and absorb its effects into $L_{1}$. We will therefore write the squared matrix element for $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$ as:
\begin{align}
    |\cM(\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta')|^2 &= \dfrac{L_{1}^2m_{\eta'}^{12}}{f_{\eta'}^8\Lambda^8}F(q_i\cdot q_j)
\end{align}
where $F(q_i\cdot q_j)$ is a complicated function of the scaled external momenta.

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[scale=0.2]{figures/two_four_eta_1.pdf}
        \caption{}
        \label{fig:two_four_eta_a}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[scale=0.2]{figures/two_four_eta_2.pdf}
        \caption{}
        \label{fig:two_four_eta_b}
    \end{subfigure}
    \caption{Example Feynman diagrams contributing to $\eta'\eta'\leftrightarrow\eta'\eta'\eta'\eta'$. Note that there are many diagrams similar to the one shown in figure (a) that we have not shown.}\label{fig:two_four_eta}
\end{figure}

As mentioned in the preamble of this appendix, we need only compute the thermally-averaged cross section for $\eta'\eta'\to\eta'\eta'\eta'\eta'$. We can then get the the thermal-average of $\sigma(\eta'\eta'\eta'\eta'\to\eta'\eta')$ via detailed balance. Explicitly, the relationship is:
\begin{align}
    n_{\mathrm{eq}}^4\expval{\sigma(4\eta'\to2\eta') v^3} = n_{\mathrm{eq}}^2\expval{\sigma(2\eta'\to4\eta') v}
\end{align}
with $n_{\mathrm{eq}}$ is the equilibrium number density of the $\eta'$. To compute $\expval{\sigma(2\eta'\to4\eta') v}$, we need to compute the expression given in Eqn.~(\ref{eqn:thermal_average_22}). We will thus need the zero temperature cross section, which is given by:
\begin{align}
    \sigma_{2\eta'\to4\eta'}(s) &= \left(\dfrac{L_1^2m_{\eta'}^{6}}{f_{\eta'}^4\Lambda^4}\right)^2
    \dfrac{1}{2\sqrt{s}\sqrt{s-4m_{\eta'}^2}}
    \int
    d\Pi_{3}d\Pi_{4}d\Pi_{5}d\Pi_{6}
    F(q_{i}\cdot q_{j})
    \delta^4\left(P-\sum_{i=1}^4 p_i\right)
\end{align}
where $d\Pi_i = \frac{d^3p_{i}}{(2\pi)^32E_i}$ and $P = p_{1} + p_2$ is the sum of the initial state momenta. As we did with the matrix element, we will factor out the mass dimensions of the invariant phase space integral by defining $q_i = p_i/m_{\eta'}$, $\epsilon_i = E_i / m_{\eta'}$ and $z = \sqrt{s}/m_{\eta'}$. Then, we can write the cross section as:
\begin{align}
    \sigma_{2\eta'\to4\eta'}(s) &= \left(\dfrac{L_1^2m_{\eta'}^{7}}{f_{\eta'}^4\Lambda^4}\right)^2
    \bar{\sigma}(z)
\end{align}
with 
\begin{align}
    \bar{\sigma}(z) &=
    \dfrac{1}{2z\sqrt{z^2-4}}
    \int
    \frac{d^3q_{3}}{(2\pi)^32\epsilon_3}
    \frac{d^3q_{4}}{(2\pi)^32\epsilon_4}
    \frac{d^3q_{5}}{(2\pi)^32\epsilon_5}
    \frac{d^3q_{6}}{(2\pi)^32\epsilon_6}
    F(q_{i}\cdot q_{j})\delta\left(Q-\sum_{i=1}^{4}q_i\right)
\end{align}
The numerical values of $\bar{\sigma}(z)$ are shown in Fig.~(\ref{fig:scaled_cross_section_24_eta}). One can see that the cross section grows (without bound) with the energy. This is a consequence of the fact that chiral perturbation theory is an effective field theory. In fact, for energies larger than $\sqrt{s} \sim 4\pi f_{\eta'}$, the chiral expansion breaks down and the theory becomes non-perturbative. With the numerical cross section in hand, we can numerically evaluate the thermally-average annihilation cross section, given by:
\begin{align}\label{eqn:thermal_average_22}
    \expval{\sigma_{2\eta'\to4\eta'} v} &= 
    \left(\dfrac{L_1^2m_{\eta'}^{7}}{f_{\eta'}^4\Lambda^4}\right)^2
    \dfrac{x}{4K^2_{2}(x)}
    \int_{4}^{N} dz z^2(z^2-4)K_{1}(xz)\bar{\sigma}(z) 
\end{align}
with $x = m_{\eta'} / T$. Notice that we have introduced a cutoff of $N$, which is the cutoff the chiral Lagrangian ($4\pi f_{\eta'}$) scaled by the $\eta'$ mass: $z_{\mathrm{max}} = 4\pi f_{\eta'}/m_{\eta'} = N$. Fig.~(\ref{fig:thermal_cross_section_24_eta}) shows the thermally-average cross section for $\eta'\eta'\to\eta'\eta'\eta'\eta'$ for various values of $N$.


\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
       \centering
        \includegraphics[width=\textwidth]{figures/scaled_cross_section_24_eta.pdf}
        \caption{}\label{fig:scaled_cross_section_24_eta}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
       \centering
        \includegraphics[width=\textwidth]{figures/thermal_cs_eta.pdf}
        \caption{}\label{fig:thermal_cross_section_24_eta}
    \end{subfigure}
    \caption{}\label{fig:cross_section_24_eta}
\end{figure}






\subsection{$\eta'\eta'\leftrightarrow \bar{\Delta}\Delta$}

I THINK THIS IS WRONG!

As mentioned in the text, we assume that the matrix element for $\eta'\eta'\to\Delta\Delta$ scales like $e^{-cN}/\Lambda$, where $c$ is a parameter representing the combinatoric penalty of constructing $N$ colors/anticolors to make $\Delta$/$\bar{\Delta}$. The squared matrix element is given by:
\begin{align}
    |\cM_{\eta'\eta'\leftrightarrow\bar{\Delta}\Delta}|^2 &= \dfrac{e^{-2cN}}{\Lambda^2}
\end{align}
Here we will focus on $\eta'\eta'\to\bar{\Delta}\Delta$. The zero-temperature cross-section is given by:
\begin{align}
    \sigma_{\eta'\eta'\to\bar{\Delta}\Delta} &=
    \dfrac{e^{-2cN}}{\Lambda^2}
    \dfrac{\sqrt{s-4m_{\Delta}^2}}{16\pi s\sqrt{s-4m_{\eta'}^2}}
    \theta(s-4m_{\Delta}^2)
\end{align}
Using Eqn.~(\ref{eqn:thermal_average_22}), we find that:
\begin{align}
    \expval{\sigma_{\eta'\eta'\to\bar{\Delta}\Delta} v} &=
    \dfrac{e^{-2cN}}{64\pi m_{\eta'}^2 \Lambda^2}
    \dfrac{x_{\eta'}}{K_{2}(x_{\eta'})^2}
    \int_{2r}^{\infty}\dd{z}
    \sqrt{z^2-4}\sqrt{z^2-4r^2}K_{1}(x_{\eta'}z)
\end{align}
where $x_{\eta'} = m_{\eta'}/T_{d}$, $r=m_{\Delta}/m_{\eta'}$, and the new integration variable is $z=\sqrt{s}/m_{\eta'}$. To a good approximation, we since $r \sim N^{3/2}$ is large, we can replace $\sqrt{z^2-4}$ with $z$ and integrate this expression exactly. The result is:
\begin{align}
    \expval{\sigma_{\eta'\eta'\to\bar{\Delta}\Delta} v} &=
    \dfrac{r^2e^{-2cN}}{32\pi m_{\eta'}^2 \Lambda^2}
    \qty(\dfrac{K_1(rx_{\eta'})}{K_2(x_{\eta'})})^2
\end{align}


\acknowledgments

LM and SP are partly supported by the U.S.\ Department of Energy grant number de-sc0010107.

%\paragraph{Note added.} This is also a good position for notes added
%after the paper has been written.

\bibliographystyle{JHEP.bst}
\bibliography{references}

\end{document}

